CAPRI-Net: Learning Compact CAD Shapes with Adaptive Primitive Assembly

We introduce CAPRI-Net, a neural network for learning compact and interpretable implicit representations of 3D computer-aided design (CAD) models, in the form of adaptive primitive assemblies. Our network takes an input 3D shape that can be provided as a point cloud or voxel grids, and reconstructs it by a compact assembly of quadric surface primitives via constructive solid geometry (CSG) operations. The network is self-supervised with a reconstruction loss, leading to faithful 3D reconstructions with sharp edges and plausible CSG trees, without any ground-truth shape assemblies. While the parametric nature of CAD models does make them more predictable locally, at the shape level, there is a great deal of structural and topological variations, which present a significant generalizability challenge to state-of-the-art neural models for 3D shapes. Our network addresses this challenge by adaptive training with respect to each test shape, with which we fine-tune the network that was pre-trained on a model collection. We evaluate our learning framework on both ShapeNet and ABC, the largest and most diverse CAD dataset to date, in terms of reconstruction quality, shape edges, compactness, and interpretability, to demonstrate superiority over current alternatives suitable for neural CAD reconstruction.

==> Tables/3d_ablation.tex <==

\setlength{\tabcolsep}{4pt}
\begin{table}[h!]
\caption{Ablation study on ABC; see texts for descriptions. }
\centering
 \begin{tabular}{l r r r r r r}
     %\toprule
 Methods & CD & NC & ECD & LFD & \#P & \#C \\
    \midrule
        \addlinespace[5pt]
%AtlasNet& 0 & 0& 0 & 0 \\
w.o QS & 0.34 & 0.89 & 5.290 & 1477.3 & 71.98 & 5.06\\
w.o Diff & 0.29 & 0.86 & 4.408 & 1323.8 & 77.30 & 10.42\\
w.o Weight & 0.26 & 0.89 & 5.315 & 1047.1 & 58.44 & 5.30\\
Ours & 0.15 & 0.91 & 4.267 & 750.3 & 48.96 & 5.46\\
  %\bottomrule
\end{tabular}
    \label{tab:3d_ablation}
\end{table}


==> app.tex <==
\section{Application}
\label{sec:result}

We demonstrate generalization ability by performing two applications: single image reconstruction and incomplete point cloud surface reconstruction.

\subsection{Single view reconstruction (SVR)}



%\input{Tables/3d_shapenet_svr_quan}

\begin{figure}
  \includegraphics[width=0.9\linewidth]{figure/TBD.png}
  \caption{Single view reconstruction: 3D visual comparison in ShapeNet dataset.}
  \label{fig:3d_shapenet_svr_visual}
\end{figure}

\subsection{Incomplete point cloud completion}



\input{Tables/3d_pc_quan}

\begin{figure}
  \includegraphics[width=0.9\linewidth]{figure/TBD.png}
  \caption{Incomplete point cloud completion: 3D visual comparison in ShapeNet dataset.}
  \label{fig:3d_shapenet_ipc_visual}
\end{figure}


==> supp_main.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article} 

% \usepackage{iccv}
% \usepackage{times}
% \usepackage{epsfig}
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb,bm}
% \usepackage{booktabs}
% \usepackage{mathrsfs}
% \usepackage[T1]{fontenc}
% \usepackage{textcomp}
% \usepackage{bbm}
% Include other packages here, before hyperref.

% If you comment hyperref and then uncomment it, you should delete
% egpaper.aux before re-running latex.  (Or just hit 'q' on the first latex
% run, let it finish, and you should be clear).
% \usepackage[pagebackref=true,breaklinks=true,letterpaper=true,colorlinks,bookmarks=false]{hyperref}


% \iccvfinalcopy % *** Uncomment this line for the final submission

\def\iccvPaperID{5432} % *** Enter the ICCV Paper ID here
\def\httilde{\mbox{\tt\raisebox{-.5ex}{\symbol{126}}}}

% Pages are numbered in submission mode, and unnumbered in camera-ready
%\ificcvfinal\pagestyle{empty}\fi

%\input{ourcommands}
% \begin{document}

%%%%%%%%% TITLE
%\title{CAPRI-Net: Learning Compact CAD Shapes with Adaptive Primitives}
\title{CAPRI-Net: Learning Compact CAD Shapes with Adaptive Primitive Assembly}

\author{First Author\\
Institution1\\
Institution1 address\\
{\tt\small firstauthor@i1.org}
% For a paper whose authors are all at the same institution,
% omit the following lines up until the closing ``}''.
% Additional authors and addresses can be added with ``\and'',
% just like the second author.
% To save space, use either the email address or home page, not both
\and
Second Author\\
Institution2\\
First line of institution2 address\\
{\tt\small secondauthor@i2.org}
}

\maketitle
% Remove page # from the first page of camera-ready.
%\ificcvfinal\thispagestyle{empty}\fi

%%%%%%%%% ABSTRACT
\input{supp}
%\input{points}


% % \clearpage
% \newpage
% \onecolumn
% {\small
% \bibliographystyle{ieee_fullname}
% \bibliography{ref}
% }

% \end{document}
